Deep Kalman Filters

Kalman Filters are one of the most influential models of time-varying phenomena. They admit an intuitive probabilistic interpretation, have a simple functional form, and enjoy widespread adoption in a variety of disciplines. Motivated by recent variational methods for learning deep generative models, we introduce a unified algorithm to efficiently learn a broad spectrum of Kalman filters. Of particular interest is the use of temporal generative models for counterfactual inference. We investigate the efficacy of such models for counterfactual inference, and to that end we introduce the "Healing MNIST" dataset where long-term structure, noise and actions are applied to sequences of digits. We show the efficacy of our method for modeling this dataset. We further show how our model can be used for counterfactual inference for patients, based on electronic health record data of 8,000 patients over 4.5 years.

==> joint_kl.tex <==

%
\section{Joint distribution of Prior\label{sec:prior}}
In this section, we detail the form of the prior distribution over latent variables for a Kalman Filter
whose distribution is given as:

\begin{align*}
	&Z_1\sim \Normal(0;\Id)\\	
	&Z_t\sim\Normal(Z_{t-1}+U_{t-1}|\dt_t\Id)\quad\forall t\in2\ldots T\\
	&X_t \sim P(X_t|Z_t) \quad\forall t
\end{align*}

Where $X_1\ldots X_T$ are the observations, $Z_1\ldots Z_T$ are the latent variables and $U_1\ldots U_T$
represent embeddings of external noise variables at every time step. $P(X_t|Z_t)$ is parameterized by a neural
network. $\dt_t\Id$ is the scaled identity where $\dt_t$ represents the amount of time passed between 
consecutive observations. For simplicity, moving forward, we assume a constant $\dt$. 

\textbf{Role within the Patient-Doctor Model}
Here, the latent variables $Z$ can be used to model the doctor's latent state 
and equivalently the patients latent state. 
In the case of the former, the variables $U_t$ represent embeddings
of the observations generated from the patient's latent variables into the space spanned that the doctor. 

The prior distribution is $p(Z_1\ldots Z_T|U_1\ldots U_{T-1}) = p(Z_1)\prod_{t=2}^T p(Z_t|Z_{t-1},U_{t-1})$ 
where. While the joint distribution factorizes, 
with each element a Gaussian, 
we seek to compute the density of the distribution of the concatenated vector $[Z_1\ldots Z_T]$.
We assume $Z_t$ are $D$ dimensional vectors.

Recall the form of a multivariate Normal:
\begin{align*}
p(Y) = &\Normal(\mu;\Sigma)\\ 
	= &\exp\left(-\frac{1}{2}(Y-\mu)^T\Sigma^{-1}(Y-\mu)-\frac{D}{2}\log 2\pi -\frac{1}{2}\log\Sigma\right)
\end{align*}
For some scalar $\dt$, we have that $\log\det(\dt \Id) = D \log\dt$.
We describe the joint for $T=2$ and $T=3$, the pattern
that forms is obvious:

\begin{align*}
p(Z_1,Z_2) &= p(Z_1)\pt{2}{1}\\
	&= \Normal(0,\Id) \distt{1}\\
	&= \exp(-D\log 2\pi + \frac{D}{2} \log\dt \\ 
	&-(\underbrace{\frac{Z_1^TZ_1}{2} + \frac{\dt}{2}(Z_2-(Z_1+U_1))^T(Z_2-(Z_1+U_1))}_{(a)}))\\ 
\end{align*}

Since, the sum of two quadratic forms continues to be quadratic, we simplify $(a)$ 
as follows:
\begin{dmath*}
\frac{Z_1^TZ_1}{2} +\frac{\dt}{2}(Z_2-(Z_1+U_1))^T(Z_2-(Z_1+U_1)) = \frac{Z_1^TZ_1}{2} + \frac{\dt}{2}(Z_2^TZ_2 + Z_1^TZ_1 + U_1^TU_1 -2Z_2^TZ_1 -2Z_1^TU_1 -2Z_2^TU_1)
= \frac{1}{2}(\cattwo{Z_1}{Z_2} - \cattwo{0}{U_1})^T \begin{bmatrix} (1+\dt)\Id &-\dt\Id \\ -\dt\Id &\dt\Id\end{bmatrix} (\cattwo{Z_1}{Z_2} - \cattwo{0}{U_1}) 
\end{dmath*}

Therefore, we have that 
\begin{dmath*}
p(\cattwo{Z_1}{Z_2}) = \exp(-D\log 2\pi + \frac{D}{2} \log\dt \\
-\frac{1}{2}(\cattwo{Z_1}{Z_2} - \cattwo{0}{U_1})^T \\
\begin{bmatrix} (1+\dt)\Id &-\dt\Id \\ -\dt\Id &\dt\Id\end{bmatrix} (\cattwo{Z_1}{Z_2} - \cattwo{0}{U_1})
\end{dmath*}
Note that this is a normalized Gaussian of dimension $2D$ with $\mu = \cattwo{0}{U_1}$ and $\Sigma^{-1} =  \begin{bmatrix} (1+\dt)\Id &-\dt\Id \\ -\dt\Id &\dt\Id\end{bmatrix}$.

We can also show that: $ \log\det\Sigma^{-1} = D \log \dt$.
This can be computed using Schur's Complement: for a matrix $M=\begin{bmatrix}A&B\\C&D\end{bmatrix}$, $\det M = \det D\det(A -  BD^{-1}C)$. Taking $A = (1+\dt)\Id, B = -\dt\Id, C = -\dt\Id, D = \dt\Id$, we get that $\det \Sigma^{-1} = \det (\dt\Id)\det ((1+\dt)\Id - \dt \Id) = \dt^{D}$.
This immediately gives us the desired form for $\log\det\Sigma^{-1}$.

We now consider the case of $T=3$. Here we have that 

\begin{dmath*}
	p(Z_1,Z_2,Z_3) = \pt{3}{2}p(Z_1,Z_2) 
= \exp\left(-\frac{3D}{2}\log 2\pi + \frac{2D}{2} \log\dt\\
-( \cattwo{Z_1}{Z_2} - \cattwo{0}{U_1})^T \begin{bmatrix} (1+\dt)\Id &-\dt\Id \\ -\dt\Id&\dt\Id \end{bmatrix}\\
(\cattwo{Z_1}{Z_2} - \cattwo{0}{U_1}) + \frac{(Z_3-Z_2-U_2)^T(Z_3-Z_2-U_2)}{2} \right)
= \exp\left(-\frac{3D}{2}\log 2\pi + \frac{2D}{2} \log\dt + (\catthr{Z_1}{Z_2}{Z_3}-\catthr{0}{U_1}{U_1+U_2})^T \\
\begin{bmatrix}  (1+\dt)\Id &-\dt\Id & 0 \\  -\dt\Id&2\dt\Id& -\dt\Id \\0&-\dt\Id&\dt\Id \end{bmatrix} (\catthr{Z_1}{Z_2}{Z_3}-\catthr{0}{U_1}{U_1+U_2})\right)
\end{dmath*}

This is a Gaussian of dimension $3D$ with mean $\catthr{0}{U_1}{U_1+U_2}$ and $\Sigma^{-1} = \begin{bmatrix}  (1+\dt)\Id &-\dt\Id & 0 \\  -\dt\Id&2\dt\Id& -\dt \Id\\0&-\dt\Id&\dt\Id \end{bmatrix}$


\todo[inline]{Generalize using inductive argument}
Therefore, in the general case, we have that:
\begin{dmath}
	\label{eqn:prior}
	p([Z_1\ldots\;Z_T]) = \mathcal{N}\left(\mu_p| \Sigma_p\right)
\end{dmath}
where $\mu_p = [0\;U_1\;U_1+U_2\;\ldots\;\sum_{t}U_t]$ and $\Prec{p}$ is a tridiagonal matrix with the diagonal given by $[(1+\dt)\Id\;2\dt\Id \;2\dt \Id \;\ldots\;2\dt \Id \;\dt \Id]$ 
and the upper and lower diagonal comprising $-\dt\Id$. 


%
\section{Computing the KL divergence\label{sec:kldiv}}

The KL divergence between two multivariate Gaussians can be written as:
\begin{dmath*}
	KL(q||p) = \frac{1}{2}\left( \underbrace{\log\frac{|\Sigma_p|}{|\Sigma_q|}}_{(a)} -D + \\
	\underbrace{\Tr(\Prec{p}\Sigma_q)}_{(b)} + \underbrace{(\mu_p-\mu_q)^T\Prec{p}(\mu_p-\mu_q)}_{(c)}\right)
\end{dmath*}
The choice of $q$ and $p$ is suggestive. Using the result of Section \ref{sec:prior}, we can write the 
analytic form for the KL divergence of two Gaussians.

Since we use a fully factorized variational posterior, we have that:
$$q([X_1\;X_2\;\ldots\;X_T]) = \mathcal{N}(\mu_q|\Sigma_q)$$
where $\mu_q = [\mu_{q1}\;\mu_{q2}\;\ldots\;\mu_{qT}]$ and $\Sigma_q = blkdiag([\Sigma_{q1}\;\Sigma_{q2}\;\ldots\;\Sigma_{qT}])$.
The form of the inverse covariance for the Gaussian $p$ is given by Equation \ref{eqn:prior}.

\textbf{Term (a)}
\begin{dmath*}
	\log\frac{|\Sigma_p|}{|\Sigma_q|} = - (-\log|\Sigma_p|) -\log |\Sigma_q|\\
	= -(\log |\Prec{p}|) -\log\prod_{t=1}^T |\Sigma_{qt}|\\
	= -(T-1)\cdot D \cdot log(\dt) - \sum_{t=1}^T \log|\Sigma_{qt}|\\
\end{dmath*}

\textbf{Term (b)}

Here we use the identity $\Tr(AB^{T}) = \sum_{ij} A_{ij}B_{ij}$, the fact that $\Sigma_q$ is block diagonal and $\Prec{p}$ is block tri-diagonal with each block comprising scaled $\Id$ matrices.
\begin{dmath*}
	\Tr(\Prec{p}\Sigma_q) = (1+\dt)\Tr\Sigma_{q1} + 2\dt\sum_{t=2}^{T-1}\Tr\Sigma_{qt} + \dt\Tr\Sigma_{qT} 
\end{dmath*}


\textbf{Term (c)}

The quadratic form based on the non-zero elements of the symmetric $\Prec{p}$ realizes two sets of terms. One from the main diagonal and the other (symmetric) terms from the upper and lower diagonal.

\begin{dmath*}
	(\mu_p-\mu_q)^T\Prec{p}(\mu_p-\mu_q) = (1+\dt)\normtwo{\mu_{q1}}^2 
	+ 2\dt\sum_{t=2}^{T-1}\normtwo{\sum_{i=1}^{t-1}U_i - \mu_{qt}}^2 + \dt\normtwo{\sum_{i=0}^{T-1}U_i-\mu_{qT}}^2
	\\
	+2\left[-\dt\sum_{t=2}^{T} \left(\sum_{i=0}^{t-2}U_i - \mu_{q(t-1)}\right)^T \left(\sum_{i=0}^{t-1}U_i-\mu_{qt}\right)\right]
\end{dmath*}

Denoting $b^{t} = \sum_{i=1}^t U_i$, we have:

\begin{dmath}
	KL(q||p) = \frac{1}{2}\left\{-(T-1)\dt - \sum_{t=1}^T \log|\Sigma_{qt}| -TD \\
	+(1+\dt)\Tr\Sigma_{q1} + 2\dt\sum_{t=2}^{T-1}\Tr\Sigma_{qt} + \dt\Tr\Sigma_{qT}\\
	+(1+\dt)\normtwo{\mu_{q1}}^2+ 2\dt\sum_{t=2}^{T-1}\normtwo{b^{t-1} - \mu_{qt}}^2 + \dt\normtwo{b^{T-1}-\mu_{qT}}^2 \\
	+\left[-2\dt\sum_{t=2}^{T} \left(b^{t-2}- \mu_{q(t-1)}\right)^T \left(b^{t-1}-\mu_{qt}\right)\right] \right\} 
\end{dmath}

\begin{comment}
\section{Gradients of the KL divergence\label{sec:grad_KL}}
We detail the form of the gradients of the KL divergence. In the simplest setting,
we represent $\Sigma_{qt}$ using a diagonal covariance matrix. 
We parameterize a neural network to represent this diagonal with the vector 
representing: $\lgsigsq$. The mean vector is parameterized directly.

\textbf{Gradients with Respect to $\mu_{qt}$}

\begin{dmath}
	\nabla_{\mu_t} KL(q||p) = \\
	\frac{1}{2}\left(\Ind{t=1}2(1+\dt)\mu_{q1} + \Ind{t=T}2\dt (\mu_{qT}-b^{T-1})\\ 
	+ \Ind{1<t<T}4\dt (\mu_{qt}-b^{t-1})\\
	+\dt \Ind{t=1} (b^1-\mu_{q2})\\
	+\dt \Ind{t=T} (b^{T-2}-\mu_{q(T-1)})\\
	+\dt \Ind{1<t<T}\left((b^{t-2}-\mu_{q(t-1)}) + (b^t-\mu_{q(t+1)})\right)
	\right) 
\end{dmath}

\textbf{Gradients with respect to $\lgsigsq$}
We can rewrite the terms in the KL that depend on $\Sigma_{qt}$ based on 
a parameterization given by $k_t = \lgsigsq_t$ as follows:

\begin{dmath}
	KL(q||p)_{k_t} = \\
	\frac{1}{2}\left\{ -\sum_{t=1}^{T} k_t  + 
\Ind{t==1}(1+\dt)\exp(0.5k_t) + \\
\Ind{t==T}\dt\exp(0.5k_t) + \Ind{1<t<T}2\dt\exp(0.5k_t)\right\}
\end{dmath}
\begin{dmath}
	\nabla_{k_t} KL(q||p) \\
	= \frac{1}{2}\left\{-1 +\Ind{t=1}(1+\dt)\exp(0.5k_t)*0.5 + \\
	\Ind{t=T}\dt\exp(0.5k_t)*0.5 + \Ind{1<t<T}2\dt\exp(0.5k_t)*0.5\right\}
\end{dmath}

\textbf{Gradients with respect to $U_{t}$}

$U_t$ is an embedding into the latent space of $Z$. 
This embedding is obtained as an output from
a neural network. 

\textit{Part (A)}

When $k= T-1$, 
$U_{T-1}$ appears in $\dt||b^{T-1}-\mu_{qT}||^2_2$
and $\nabla_{U_{T-1}} KL(q||p) = 2\dt (b^{T-1}-\mu_{qT})$
where we used $\frac{d b^t}{d U_{k}} = 1$ for $1\leq k\leq t$ and $0$ otherwise.

\textit{Part (B)}

For $1\leq k\leq T-1$, we have that $U_{k}$ appears in:

\begin{dmath*}
  \underbrace{2\dt\sum_{t=2}^{T-1}||b^{t-1}-\mu{qt}||_2^2}_{(a)}\\ 
  -2\dt\sum_{t=2}^{T}\underbrace{(b^{t-2}-\mu_{q(t-1)})^T}_{(b)}
  \underbrace{(b^{t-1}-\mu_{qt})^T}_{(c)}\\ 
\end{dmath*}

Case (i) Gradient due to Term (a)

This comprises a sum of terms where $U_k$ appears for $t\geq k+1$

$$\nabla_{U_k} KL(q||p)_{(i)} = 4\dt\sum_{t=k+1}^{T-1} (b^{t-1}-\mu_{qt})$$ 

Case (ii) Gradient when $U_k$ appears in Term (c) but not Term (b) 

$$\nabla_{U_k} KL(q||p)_{(ii)} = -2\dt (b^{k-1}-\mu_{qk})$$ 

Case (iii) Gradient when $U_k$ appears in Term (b) and Term (c)

For convenience, we define $b^k_j = b^l-U_j$

We can therefore write a single expression in term (b) and (c) as:

\begin{dmath*}
	(b^{t-2}_k +U_k -\mu_{q(t-1)})(b^{t-1}_k +U_k -\mu_{qt})\\
	\implies (U_k^TU_k + U_k^T(b^{t-2}_k+b^{t-1}_b -\mu_{qt}-\mu_{q(t-1)}))
\end{dmath*}

Taking gradients of this single expression with respect to $U_k$ yields:
\begin{dmath}
  \label{eqn:grad_single_term_part_bc}
	2U_k + b^{t-2}_k+b^{t-1}_b -\mu_{qt}-\mu_{q(t-1)}\\
	\implies b^{t-2}-\mu_{q(t-1)} + b^{t-1}-\mu_{qt}
\end{dmath}

If $U_k$ appears in both Term (b) and (c), it means that $t\geq k+2$, therefore 
using \eqref{eqn:grad_single_term_part_bc} and summing up from $t=k+2\ldots T$, we get that:

\begin{dmath*}
  \nabla_{U_k}KL(q||p)_{(iii)} = 	-2\dt \left[ \sum_{t=i+2}^{T-1}b^{t-2}-\mu_{q(t-1)} \\
  +\sum_{t=i+2}^{T-1} b^{t}-\mu_{qt}\right]\\
  =  -2\dt \left[ 2\sum_{t=k+1}^{T-1} (b^{t-1}-\mu_{qt}) -(b^k-\mu_{q(k+1)})\right] 
\end{dmath*}

In the above, we applied a change of variable to the first summation and added and subtracted
$b^{k}-\mu_{q(k+1})$ to the second summation. 

Adding up the gradients for the three cases, we get:
\begin{dmath}
  \nabla_{U_k} KL(q||p) = 4\dt\sum_{t=k+1}^{T-1} b^{t-1}-\mu_{qt} \\
  		-2\dt(b^{k-1}-\mu_{qk}) +2\dt(b^{k}-\mu_{q(k+1)})\\
		-4\dt\sum_{t=k+1}^{T-1} b^{t-1}-\mu_{qt}\\
		= 2\dt (b^{k}-b^{k-1}-(\mu_{k+1}-\mu_{qk}))\\
		= 2\dt (U_k - (\mu_{k+1}-\mu_{qk}))\\
\end{dmath}


The implication of this is that the role of the embedding function used to map to $U_t$ is
to match the difference between means in the posterior distribution of consecutive latent
variables. 

%
\begin{comment}
\textit{Part (i)}

Consider the gradients with respect to the function: 
$$K = 2\dt\sum_{t=2}^{T-1}||b^{t-1}-\mu_{qt}||^2_2 + \dt||b^T-\mu_{qT}||^2_2$$

\begin{dmath}
	\nabla_{a_i} K = 2\dt(b^{T-1}-\mu_{qT}) + 4\dt\sum_{t=i+1}^{T-1}(b^{t}-\mu_{qt})
\end{dmath}

\textit{Part (ii)}

Now consider the gradients with respect to the function:

$$K = -\dt \sum_{t=2}^T \left(b^{t-2}-\mu_{q(t-1)}\right)^T \left(b^{t-1}-\mu_{qt}\right)$$

When $t=T$, the gradients of this function are simply: 
$-\dt(b^{T-2}-\mu_{q(T-1)})$

For $1\leq t< T$, we consider two cases. 

$t= i +1$ is the first time $a_i$ appears in the above function . In this case, it appears as a linear
term for which the gradient is:
\begin{dmath}
	\nabla_{a_i} K_1 = -\dt (b^{t-2} - \mu_{q(t-1)})|_{t=i+1}  
\end{dmath}

For $t\geq i+2$, we have that $a_i$ appears in both terms of the vector product. 
For a single such value of $t$, we have that $K_t = (b^{t-2} - \mu_{q(t-1)})^T(b^{t-1}-\mu_{qt}) = (a_i + \tilde{b}^{t-2}_i - \mu_{q(t-1)})^T (a_i + \tilde{b}_i^{t-2}+a_{t-1}-\mu_{qt})$.

We can open this expression to yield:

$$a_i^Ta_i + 2\tilde{b}_i^{t-2}a_i + a_{t-1}a_i -\mu_{qt}^Ta_i - \mu_{q(t-1)}a_i + const$$

Taking derivatives with respect to $a_i$, we get:

$$2a_i + 2\tilde{b}_i^{t-2} + a_{t-1} -\mu_t -\mu_{t-1}$$

This can be simplified to yield: 

$$b^{t-2}+b^{t-1} -\mu_t -\mu_{t-1}$$

Taking the sum of the above over $i+2\leq t\leq T-1$ we get:

$$\nabla_{a_i} K_2 = \sum_{t=i+2}^{T-1}b^{t-2}+b^{t-1} -\mu_t -\mu_{t-1} = \sum_{t=i+1}^{T-1} b^{t}-\mu_{qt} + \sum_{t=i+2}^{T-1} b^t -\mu_{qt} - \sum_{t=i+2}^{T-1} a_{t-1}+a_t $$

Defining $\diff_{a}^{b} = \sum_{l = a}^{b} b^l-\mu_{ql}$
Combining $K_1$ and $K_2$, we get that the gradients with respect to $a_i$ are:
\begin{dmath}
	\nabla_{a_i} K(q||p) = \frac{1}{2} \left( 2\dt(b^{T-1}-\mu_{qT}) +4\dt \diff_{i+2}^{T-1} - \Ind{t=T}(\dt(b^{T-2}-\mu_{q(T-1)})) \\
	\Ind{1\leq t<T}(-\dt(b^{i-1}-\mu_{qi}) +\diff_{i+1}^{T-1} +\diff_{i+2}^{T-1} - \sum_{t = i+2}^{T-1} a_{t-1}+a_t )				
				\right)
\end{dmath}
\end{comment}

%
\end{comment}
\section{Maximum Likelihood Learning and Parameter Estimation}
\todo[inline]{Needs to be cleaned up}
For simplicity of notation, we interpret the latent variable $X^a_1\ldots X^a_T$ as the patient and rename them $p_1\ldots p_T$.
Similarly, we denote the other actor's latenty variable by $d_1\ldots d_T$, representing the doctor. The actions $a_1\ldots a_T$ 
are generated by the doctor and the observations $o_1\ldots o_T$ are generated by the patient.

Our goal is to learn a model of the observations ($o_1\ldots o_T$) and actions ($a_1\ldots a_T$).
The optimization problem of interest is: 

\begin{dmath*}
\max_{\theta_d,\theta_p} p(\vec{a},\vec{o}) = \max_{\theta_d,\theta_p} \int_{d,p} p(\vec{a},\vec{o},\vec{d},\vec{p})
\end{dmath*}

We simplify $p(\vec{a},\vec{o},\vec{d},\vec{p})$ as follows:

\begin{dmath*}
	p(\vec{a},\vec{o},\vec{d},\vec{p}) = p(p_1)\prod_{t=2}^T p(p_t|p_{t-1},a_{t-1}) \prod_{t=1}^T p(o_t|p_t) \;\;p(d_1)\prod_{t=2}^T p(d_t|d_{t-1},o_{t-1})\prod_{t=1}^T p(a_t|d_t)
\end{dmath*}

\todo[inline]{This requires a proof by induction in time. Hard to prove in one step.}

For $T=2$, the relevant steps for the \textit{doctor} are:
\begin{dmath*}
	p(d_1)p(d_2|d_1,o_1)p(a_1|d_1)p(a_2|d_2) = p(d_1) p(d_2,a_1|d_1,o_1) p(a_2|d_2)\\
		= p(d_1,d2,a_1|o_1) p(a_2|d_2) \\
		= p(d_1,d_2,a_1,a_2|o_1) \\
\end{dmath*}

Therefore we find that $\max_{\theta_d,\theta_p} p(\vec{a},\vec{o}) = p_{\theta_d}(a|o) p_{\theta_p}(o|a)$
and that the two Kalman Filters may be trained separately.


==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

\tikzset{>={triangle 45}}

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->,#1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->,#1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

